Searching for chemo-kinematic structures in the Milky Way halo with deep clustering algorithms

According to the lambda CDM scenario, galaxies are formed through the hierarchical accretion of building blocks. Our Galaxy is a privileged place to look for the remnants of accretion events through the study of the chemical and kinematic properties of its halo stellar populations. Due to its low density, the stellar halo holds the most favorable conditions for chemical tagging. However, chemical tagging alone often yields weak results due to both uncertainties in chemical abundances and to overlapping chemical properties among different populations. To overcome this problem, the use of chemical and kinematic properties can be combined. In this Thesis, we developed a machine learning algorithm, named the CREEK, which combines orbital and chemical properties of halo stars observed by two large public spectroscopic surveys, Gaia-ESO and APOGEE. The CREEK operates as follows: 1)Data selection: We selected halo stars from the APOGEE and Gaia-ESO surveys based both on their velocity and metallicity and we computed their orbital parameters. 2)Using kinematics: The selected data were passed to a Siamese Neural Network that established links between stars based on their kinematic similarities. 3)Using chemistry: The graph was passed through a Graph Neural Network (GNN) auto-encoder that took as input the selected abundances. The abundances were chosen to maximize homogeneity within stars from the same cluster while ensuring distinctiveness between stars from different clusters. Additionally, we prioritised elements with smallest errors. The GNN auto-encoder computed a mean of the abundances of all connected stars, weighted on the number of links of each star and mapped the chemical space into a more efficient representation in the latent space. 4)Recovering structures: Finally, OPTICS was applied to the latent space, providing groups based on the chemical similarities of the stars.

==> OLD/2.1-Optics+Elements.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Togliere? Spostare?
\begin{comment}

    
When we apply OPTICS to our data, we are able to recognise the big differentiation between the LMg and the HMg, using [Fe/H] and [Mg/Fe] as chemical space in which to compute distances. These sequences are recovered with the following parameters: min\_samples=10, xi=0.0005, min\_cluster\_size=40, metric = 'manhattan'. The high value for the minimum cluster size is used only to save time. 

Let us now search for clusters more in detail and apply OPTICS to a restricted sample of our clusters: for almost all elements M 22, NGC 3201 and M 5 have quite compact abundance ratios. We exclude in our first selection Aluminum because it shows a strong bimodality within the cluster, as we can see in Figure \ref{fig:abuclusterAl}.
In this case, we manage to recover 2 clusters, with hyperparameters  min\_sample: 8, xi: 0.008, min\_cluster\_size=10, metric = 'manhattan'. This could be due to a problem of dimensionality: when we work in a multi-dimensional space, every value tends to be extreme in a dimension and distances tend to flatten all to the same values. To solve this problem, known as 'curse of dimensionality', there are algorithms to reduce the dimensionality of the problem.

To recover all three clusters, we implement a script that iterates over different values of min\_samples and different values of xi and search for the maximum number of clusters recovered.
 min\_sample: 5
 xi: 0.002
 Clusters recovered: 3
 Using elements Fe/H, Mg/FE, Ni/Fe, O/Fe we manage to recover all 3 clusters!!! This can be used for training. But if I try it for all clusters I get a smaller value than before: where I used to get 2 cluster, I now get 1. Check if it is normal.
 The reachability plot for this is in Figure \ref{fig:Reachplot3clusters}.
 
 \begin{figure}[H]
\centering
\includegraphics[width=0.8\textwidth]{Immagini/Reach_plot3clusters.png}
\caption{\label{fig:Reachplot3clusters} Spread of Al within the clusters, useful to select ideal clusters for the training}
\end{figure}
    
\end{comment}




